Experimental Demonstration of Attosecond Pump-Probe Spectroscopy with an X-ray Free-Electron Laser

Pump-probe experiments with sub-femtosecond resolution are the key to understanding electronic dynamics in quantum systems. Here we demonstrate the generation and control of sub-femtosecond pulse pairs from a two-colour X-ray free-electron laser (XFEL). By measuring the delay between the two pulses with an angular streaking diagnostic, we characterise the group velocity of the XFEL and demonstrate control of the pulse delay down to 270 as. We demonstrate the application of this technique to a pump-probe measurement in core-excited para-aminophenol. These results demonstrate the ability to perform pump-probe experiments with sub-femtosecond resolution and atomic site specificity.

==> authors.tex <==
\author{Zhaoheng Guo*}
\author{Taran~D.~Driver*}
\author{Sandra~Beauvarlet}

%TMO
Ming-Fu Lin
Andrei Kamalov
Peter Walter
Razib Obaid
Xiang Li
Xinxin Cheng
Thomas Wolf
Mike Glownia
Ruaridh Forbes
Matthias Kling
Kirk A. Larsen

%Chem. Sci. PULSE
Anna Wang
Jun Wang
Erik Isele
Jordan O'Neal
Emily Thierstein
Phil Bucksbaum

%AD
Siqi Li
Paris Franz
David Cesar
Joe Duris
Zhen Zhang
Nick Sudar
River Robles

%CFEL
Ludger Inhester

%Campaign (for the 300/600 data)
Nora Berrah

(Imperaial)
Jon Marangos
Vitali Averbukh
Oliver Alexander
Marco Ruberti

(Universidad Autonoma de Madrid) % Fernando said no
Gilbert Grell
Solene Oberli
Fernando Martin
Antonio Picon
Alicia Palacios

(Paul Scherrer Institut)
Christoph Bostedt
Andre Al-Haddad % Andre said no

(The Ohio State University)
Greg McCracken  % Haven't replied yet
Daniel Tuthill
Lou DiMauro
Zifan Wang  % Waiting for Lou's reply

(Tohoku University)
Kiyoshi Ueda

(Argonne National Lab)
Gilles Doumy
Linda Young

(Lawrence Berkeley National Lab)
Oliver Gessner
Daniel Slaughter
Thorsten Weber

(Kansas State University)
Daniel Rolles
Artem Rudenko

\author{Nora Berrah}
\affiliation{}
\author{James~P.~Cryan}
\affiliation{}
\author{Agostino~Marinelli}
\affiliation{}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
